STiTch: Semantic Transition and Transportation in Collaboration for Training-Free Zero-Shot Composed Image Retrieval

Training-free zero-shot composed image retrieval models are recently gaining increasing research interest due to their generalizability and flexibility in unseen multimodal retrieval. Recent LLM-based advances focus on generating the expected target caption by exploring the compositional ability behind the LLMs. Although efficient, we find that 1) the generated captions tend to introduce unexpected features from the reference image due to the semantic gap between the input image and text modification, where the image contains much more details than the text; 2) the point-to-point alignment during the retrieval stage fails to capture diverse compositions. To address these challenges, we introduce a novel Semantic Transition and Transportation in collaboration framework for training-free zero-shot CIR tasks. Specifically, given the composed caption inferred by an LLM, we aim to refine it through a transition vector in the embedding space and make it closer to the target image. Combining LLMs with user instruction, the refined caption concentrates more on the core modification intent and thus filters out unnecessary noise. Moreover, to explore diverse alignment during the retrieval stage, we model the caption and image as discrete distributions and reformulate the retrieval task as a set-to-set alignment task. Finally, a bidirectional transportation distance is developed to consider fine-grained alignments across modalities and calculate the retrieval score. Extensive experiments demonstrate that our method can be general, effective, and beneficial for many CIR tasks.

==> pvrxdxhprxfbkgzgdcbcvhwnphknnwwq/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\usepackage{ulem}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> pvrxdxhprxfbkgzgdcbcvhwnphknnwwq/sec/0_abstract.tex <==
\begin{abstract}
Training-free zero-shot composed image retrieval models are recently gaining increasing research interest due to their generalizability and flexibility in unseen multimodal retrieval. Recent LLM-based advances focus on generating the expected target caption by exploring the compositional ability behind the LLMs. Although efficient, we find that 1) the generated captions tend to introduce unexpected features from the reference image due to the semantic gap between the input image and text modification, where the image contains much more details than the text; 2) the point-to-point alignment during the retrieval stage fails to capture diverse compositions.
To address these challenges, we introduce a novel \underline{\textbf{S}}emantic \underline{\textbf{T}}rans\underline{\textbf{i}}tion and \underline{\textbf{T}}ransportation in \underline{\textbf{c}}ollaboration framework for training-free zero-s\underline{\textbf{h}}ot CIR tasks. Specifically, given the composed caption inferred by an LLM, we aim to refine it through a transition vector in the embedding space and make it closer to the target image. Combining LLMs with user instruction, the refined caption concentrates more on the core modification intent and thus filters out unnecessary noise. Moreover, to explore diverse alignment during the retrieval stage, we model the caption and image as discrete distributions and reformulate the retrieval task as a set-to-set alignment task. Finally, a bidirectional transportation distance is developed to consider fine-grained alignments across modalities and calculate the retrieval score.
Extensive experiments
demonstrate that our method can be general, effective, and beneficial for many CIR tasks.
% \footnote{Code is available at: \url{https://github.com/keepgoingjkg/STiTch}}.
\end{abstract}

% \begin{abstract}
% Test.
% \end{abstract}

==> pvrxdxhprxfbkgzgdcbcvhwnphknnwwq/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Composed Image Retrieval (CIR) aims to search for a target image using a compositional query of a reference image and text modification~\cite{vo2019composing,lee2021cosmo,hosseinzadeh2020composed,chen2020image,baldrati2022effective}. 
% By integrating multiple modalities, CIR enables more expressive and flexible queries than methods that rely solely on images or text, which often fail to fully capture the range of user preferences. For example, a user searching for a dress might upload an image showcasing their desired style and provide additional textual inputs like "blue," "knee length", or "floral pattern" to specify their preferences further. 
One of the key challenges is to model the multimodal relationship of the triplet: $<$\textit{reference image, text modification, target image}$>$. Previous studies have focused on fusing the input image and modifications within a shared embedding space in a supervised manner~\cite{vo2019composing,delmas2022artemis,anwaar2021compositional}. Generally, these models typically rely on expensive manually-annotated triplets and often exhibit suboptimal performance in unseen scenarios~\cite{baldrati2023zero,karthik2023vision}. 
Motivated by the success of textual inversion in image generation~\cite{gal2022image,mokady2023null,wang2024instruction}, recent studies have proposed Zero-Shot Composed Image Retrieval (ZS-CIR)~\cite{saito2023pic2word,zeng2022socratic,HyCIR}. These models focus on training a mapping network to convert the reference image into continuous textual embeddings and then merge them with text modifications using static templates for target captions, enabling CIR without explicit supervision. Unfortunately, these models also need image-caption pairs to learn the mapping parameters, and the mismatch between textual inversion and CIR may hamper their ability to accurately infer the implicit user intent conveyed in the text modification.

\begin{figure*}[!t]
\centering
\includegraphics[width=0.9\textwidth]{sec/Fig/motivation_v8.pdf}
\caption{\small{Motivation of our proposed model. Predicted captions from MLLMs typically consist of expected ground-truth sentences (red words) and unexpected visual details (gray words).}}
\label{motivation_1}
\vspace{-3mm}
\end{figure*}


Alternatively, training-free approaches paired with foundation models can achieve effective CIR without additional training and offer improved reasoning capabilities \cite{karthik2023vision,tang2025reason}. 
% Currently, two-stage methods leverage VLMs, such as BLIP-2 \cite{li2023blip}, to generate detailed descriptions of reference images. These descriptions, combined with the textual query, are then utilized by a large language model (LLM) to produce a caption for the desired target image. Finally, a VLM is employed to retrieve the corresponding image. 
% % However, this two-stage process, in which image captioning is conducted independently of the modification, often leads to inaccuracies 
% % % as critical visual details and implicit intent may be overlooked/
% % due to the inherent intrinsic information loss. 
% However, separating input captioning from modification in this step-by-step process often leads to inaccuracies due to inherent information loss.
% % Such limitation arises from the failure to capture nuanced interactions between multimodal components. Besides, it faces the challenge of higher memory and time costs. 
% Differently, one-stage approaches handle visual and textual queries simultaneously. 
There are mainly two directions: two-stage methods typically require an image captioner and an LLM to first generate detailed captions of the reference image and then fuse them with text modification via an LLM to produce the target descriptions; one-stage methods unify this process by employing an MLLM to directly output the target captions given the multimodal queries.
Despite considerable progress, several challenges remain. First, the above generation-then-retrieval pipeline is prone to \textit{Extraneous Cognitive Load} \cite{sweller1988cognitive}.  
Specifically, the reference image may trigger information leakage, which in turn leads to overemphasis on irrelevant details, affecting the retrieval performance. As shown in Fig.\ref{motivation_1}, the target caption generated by MLLMs includes extraneous elements such as ``red jacket and sunglasses'', which are unrelated to the textual modification. Therefore, distracting from the core intent,  it diminishes the ability to identify key information, such as ``snow-covered mountains''. 
Second, most existing models generate either a single description or simply average multiple descriptions to obtain the final representation~\cite{tang2025reason,yang2024semantic}. However, as one image is worth a thousand words, such point-to-point alignment focuses on partial features and fails to capture complex relations. This inherent heterogeneity between visual and textual representations inevitably leads to semantic imbalance across modalities, leading to suboptimal retrieval prediction~\cite{zhu2024awt,chen2023plot,wang2023tuning}. 

To address the above issues, we proposes STiTch, a novel one-stage, training-free framework that improves the existing generation-then-retrieval pipeline by introducing \underline{\textbf{S}}emantic \underline{\textbf{T}}rans\underline{\textbf{i}}tion and \underline{\textbf{T}}ransportation in \underline{\textbf{c}}ollaboration framework for zero-s\underline{\textbf{h}}ot CIR tasks. Like previous works~\cite{tang2025reason}, we explore the in-context learning of MLLMs and directly query an MLLM to generate the target caption given the reference image and text modification. Importantly, to address the above asymmetry issues, STiTch utilizes the uncertainty ability of the language decoder and views the description as a discrete distribution by generating multiple candidates. Each candidate in the distribution focuses on a specific composition pattern, and they together provide a comprehensive understanding of the given query input.
% Ideally, the result should capture both the image's visual features and the nuanced semantic relationship between the reference image and the desired descriptions from the instructions.
% a MLLM as the caption generator that takes the reference image and text modification as input, producing the expected target caption. Ideally, the composed result should accurately capture not only the visual features of the image but also the nuanced semantic relationship between the reference image and the desired descriptions, as expressed in the instructions. 
% To achieve this, we adopt a chain-of-thought strategy, using a few simple examples to naturally adapt the MLLM for deriving joint image-text information.
% Moreover, recognizing that a single composed text is insufficient, we effectively generate a variety of edited captions that encompass the diverse potential semantics of the composed results.\rr{emphasis various caption with diversity through sampling/diversity and divergence/provide a high degree of freedom to depict textual query/}
%Intuitively, a single deterministic composed text is insufficient. To enrich the captions, we utilize the MLLM decoder's sampling strategies to bring randomness and flexibility to the generation process. 
% This approach produces diverse and divergent captions, enabling richer semantic exploration and offering greater freedom to 
% % accurately and
% comprehensively represent the query.


% Moreover, it remains unclear whether to preserve visual concepts that are not mentioned in the modified text, and the localization of key visual regions is also challenging.
% Given that reference images may inevitably introduce irrelevant information into the captions generated by MLLMs, we utilize text modification as a natural corrector to transit the vanilla generated caption toward a more robust one. 


Since reference images may inevitably introduce irrelevant information into captions generated by MLLMs, we propose guiding the textual caption toward the target image via a transition vector in the embedding space (as seen in Fig.~\ref{motivation_1}). Intuitively, an ideal transition vector should bridge the semantic gap between the generated caption and the target image. Here, we aim to solve it in a training-free manner and estimate the transition vector by feeding the text modification into the CLIP text encoder.
For one thing, since both the text modification and the generated caption share the same modality, the former can seamlessly refine the latter without introducing a modality gap or requiring extra parameters. For another, the text modification encapsulates the incremental, high-quality, and dense information that shifts from the reference image to the target image, guiding the model to refocus on core semantic information. This transition operates directly in the embedding space—simple yet efficient—and ensures that the final target caption retains diversity while reducing distortion, all of which is highly relevant and beneficial to the retrieval process. 
% \rr{Operate directly in the embedding space}

% Previous work hsas overlooked the enhancement of reference image, which can also enrich the input with varied and multiscale perspectives. 
After obtaining high-quality and diverse features of target captions, it is crucial to align them more effectively with the target images in the embedding space. Similar to the textual domain, STiTch models each target image as a discrete distribution through multiple augmentations, where each captures local visuals of the target image. Together, these augmentations provide a rich visual representation from the visual domain, facilitating fine-grained alignments in the retrieval process.
% . \rr{In other words, while the visual embedding of the original image captures global semantics, the embeddings of its augmented views reveal fine-grained and diverse visual cues. Together, they facilitate a truly balanced semantic representation in the retrieval process.} 
% To complete the retrieval process, 
Finally, a novel bidirectional transportation distance is further developed to calculate the similarity of two discrete distributions across the vision-language modalities. Specifically, given the cost matrix that measures the transport cost between the captions and image augmentation, STiTch designs both a forward path and a backward path to calculate the transportation distance from the caption set to the target image set and that from the target image set back to the caption set, respectively. This formulation effectively uncovers fine-grained cross-modal correlations by minimizing the bidirectional transport cost between modalities.

% In summary, our STiTch shares the following contributions:
 The main contributions can be summarized as follows:

\begin{itemize}
    \item We propose a novel one-stage, training-free framework that considers both semantic transition and transportation collaboratively for ZS-CIR. By introducing the modification-driven transition to the generated caption, the feature drift caused by additional irrelevant noise is compensated in the embedding space.
    \item We elegantly transform the retrieval procedure into a bidirectional transport problem. Explicitly explore fine-grained alignments between diverse refined textual captions and enhanced target images.
    \item Extensive comparisons and ablations on four benchmarks demonstrate the effectiveness of the proposed STiTch with competitive performance in all settings.
\end{itemize}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
% The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please, number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for the reader to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, do not assume that the reviewers will read this material.

% Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% However, for your results, you should not identify yourself and should not mention your participation in the challenge.
% Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> pvrxdxhprxfbkgzgdcbcvhwnphknnwwq/sec/2_related_work.tex <==
\section{Related Work}
% \vspace{-3mm}
\label{sec:related_work}


\subsection{Composed Image Retrieval}
% The growing interest in Composed Image Retrieval (CIR) has
% contributed to several architectural innovations \cite{vo2019composing,chen2020image,lee2021cosmo}. Early methods train cross-modal networks using a fusion paradigm, which learns joint embeddings that combine reference image and modification features via contrastive objectives or attention mechanisms \cite{chen2020learning,anwaar2021compositional}. However, these supervised approaches are often time-consuming and lack scalability. Zero-Shot Composed Image Retrieval (ZS-CIR), a specialized variant, addresses these issues by enabling retrieval without relying on labeled triplets during training. For instance, Pic2Word\cite{anwaar2021compositional} learns a projection network to map image features into token embedding space, while SEARLE \cite{baldrati2023zero} uses a text inversion network to distill the mapping network for better alignment.
% % with nouns
% Another line of research focuses on generating extra triplet data from image-caption
% pairs using generative models\cite{gu2023compodiff}. 
Composed Image Retrieval (CIR) has inspired various architectural innovations \cite{vo2019composing,chen2020image,lee2021cosmo}. Early methods adopt a fusion paradigm to learn joint embeddings of reference image and modification features via contrastive or attention-based objectives \cite{chen2020learning,anwaar2021compositional}. Some recent works train large-scale retrieval models on millions of web-mined triplets\cite{zhang2024magiclens}, but reliance on supervision limits scalability. To address this, Zero-Shot CIR (ZS-CIR) enables retrieval without labeled data \cite{tang2025missing}. For example, Pic2Word \cite{anwaar2021compositional} projects image features into a token embedding space, while SEARLE \cite{baldrati2023zero} improves alignment via a text inversion network. Another line of work generates synthetic triplets from image-caption pairs using generative models \cite{gu2023compodiff}.

With the advent of foundation models, recent studies have tackled CIR in a training-free manner, leveraging their
% inherent 
strong contextual understanding. 
% Two prominent directions exist: two-stage approach performs reference image captioning and text manipulation independently, while one-stage approach integrates visual and textual inputs to generate the target caption simultaneously. 
Two main paradigms have emerged: two-stage methods performs reference image captioning and text manipulation separately, while one-stage methods generate target captions directly from multimodal inputs.
% integrates multimodal inputs to generate target caption simultaneously.
For example,
CIReVL\cite{karthik2023vision} initially employs pre-trained captioning models
\cite{li2023blip} to generate caption for a given image. Subsequently, it queries an LLM to refine and recompose the caption based on text modifications for text-to-image retrieval. LDRE\cite{yang2024ldre} considers diverse semantics of the CIR and generates diverse captions at the first stage, and then adopts an ensemble strategy to get the final single feature for the multiple captions.
OSrCIR\cite{tang2025reason}
uses MLLMs to infer user intent by directly processing a query pair, guided by a reflective chain-of-thought prompt.  
However, both are overwhelmed by the rich semantic information from the reference image, which may overshadow the key modifications. Different from existing LLM-based methods, our STiTch aims to refine the captions after the generation and improve semantic alignments by formulating the retrieval task as the bidirectional transportation problem.
% Leveraging multimodal enhancement and a three-step process that aligns with human cognition—query, transit, and align—our STiTch demonstrates stronger robustness against irrelevant noise and a deeper level of modality alignment
% \rr{By leveraging a three-step process—query, transit, align—that mirrors human cognition, our STiTch distinctly demonstrates superior robustness against irrelevant noise and deeper modality alignment.}
% from a distributional perspective

% \rr{add references in rebuttal}

\subsection{Alignment via Transport Distance}
Recently, Optimal Transport (OT) \cite{villani2009optimal} has been widely used for aligning distributions
% increasingly used to infer correspondences between distributions
in various domains \cite{redko2019optimal,zhao2018label,zhao2018label,lee2019hierarchical,chen2020graph,wang2023tuning,zhu2025dynamic}.
% , including unsupervised domain adaptation\cite{redko2019optimal}, label representation\cite{zhao2018label}, and cross-modal semantics\cite{lee2019hierarchical,chen2020graph}.
% OT aims to measure the
% distance between between two probability distributions by defining a cost metric that accounts for both the magnitudes of the transported masses and the distances they are moved. 
Unlike traditional distance metrics like Euclidean distance, 
% which focus on point-to-point comparisons,
OT provides a more geometrically nuanced measure that captures structural similarities between distributions.
However, it typically requires 
% optimizing the transport plan through an iterative
iterative optimization via the
Sinkhorn algorithm \cite{cuturi2013sinkhorn}, which can be time-consuming. To this end, Conditional Transport (CT) considers the transport plan based on the semantic similarity between samples from two distributions bidirectionally \cite{zheng2021exploiting}. Its flexibility allows seamless integration with deep learning frameworks, offering lower computational complexity
and better scalability, resulting in superior performance in recent alignment tasks \cite{liu2023patch,li2023patchct,li2024tsca}. For instance, \cite{tian2023prototypes} exploits transferable statistics with CT to refine biased prototypes to capture unbiased statistics within imbalanced query samples. \cite{li2023patchct} design a sparse and layer-wise CT framework to enhance interactions between visual patches and textual labels, ensuring higher semantic consistency for multi-label classification. 
Notably, CT is inherently well-suited for a key step in CIR—aligning multiple captions with target images—especially when multimodal representations are involved. Motivated by this potential, we transform the traditional point-to-point similarity measure into a minimization of CT-based distance from a distributional perspective.

==> pvrxdxhprxfbkgzgdcbcvhwnphknnwwq/sec/3_method.tex <==
\section{Method}
\label{sec:method}

\begin{figure*}[!ht]
\centering
\includegraphics[width=0.82\textwidth]{sec/Fig/QTA_framework_9.pdf}
% \vspace{-3mm}
\caption{\small{The overall framework of our method. STiTch first queries MLLMs to generate multiple captions and then refines them towards the target image via the transition vector in the embedding space. Subsequently, the refined captions and augmented target images are modeled as discrete distributions, enabling fine-grained set-to-set alignment via bidirectional transportation.}}
\vspace{-4mm}
\label{framework}
\end{figure*}


% \subsection{Preliminaries}
\noindent \textbf{Preliminaries.}
Let us denote $(x, m, y)$ as the CIR triplet \textit{$<$reference image, text modification, target image$>$}, respectively. The first two are multimodal inputs from users describing their retrieval intent. Training-free ZS-CIR aims to search a target image 
% $\yv$ 
$y$
from an image database $\mathit{Y}=\{y_n\}_{n=1}^N$ that satisfies the semantic consistency with both $x$ and $m$, without requiring additional training. Generally, existing 
% ZS-CIR
approaches
follow a generation-then-retrieval pipeline to make the final prediction. They first feed the reference image $x$ and text modification $m$ into a fusing model (such as an MLLM) to obtain the composed description of the target image, denoted as $t=\text{MLLM}(x, m)$. The retrieval score is then calculated by CLIP similarity:
\begin{equation}\label{clip}
    p(y=i|x,m) = \frac{\text{exp}(-dis(\tv, \yv_i) / \tau)}{\sum_{n=1}^N \text{exp}(-dis(\tv, \yv_n) / \tau)},
\end{equation}
where $\tv \in R^d$ and $\yv \in R^d$ are the latent features of $t$ and $y$ in CLIP space, with $d$ denotes the embedding dimension. $dis$ is the distance function and $\tau$ is the temperature parameter. $\tv$ in Eq.~\ref{clip} can be viewed as prototypes that capture reasonable visual features of $y$. To find the optimal $\tv$, recent LLM-based models develop various attempts, including two-stage generation and chain-of-thought reasoning\cite{yang2024ldre,li2025imagine,tang2025reason}. 

Despite their promising results, We find that 1) the generated description $\tv$ usually inherits the unnecessary details from the reference image, leading to suboptimal prototype learning; 2) The point estimation of $\tv$ fails to model complex composed relations, this may limit the uncertainty of $\tv$ and diminish the generalizability.

% \subsection{Querying, Transition, and Alignment}
\subsection{{Semantic Transition and Transportation}}
Starting from Eq.~\ref{clip}, we propose a novel training-free ZS-CIR framework to solve the mentioned shortcomings, as
illustrated in Fig.~\ref{framework}. Specifically, our proposed model consists of three modules: Querying, Transition, and Alignment. 
Unlike previous point estimation of $\tv$, STiTch views the composed prototype as a discrete distribution, e.g., $P_t$, over the caption space. This allows $P_t$ to focus on various possible target captions, showing higher diversity. To alleviate the issues of unnecessary information pollution, we further transfer the obtained $\tv$ using the text modification $\mv$ in the embedding space. $\mv$ contains high-quality relative information linking the reference image to its target image. Thus, a simple combination strategy is developed to push $\tv$ to its target image, resulting in more precise $\tv$. Finally, we also view the target image as a discrete distribution and develop a bidirectional transportation distance to align the composed prototypes and target images for fine-grained retrieval. 

% \vspace{-5mm}
\noindent \textbf
% \paragraph
{Querying.} As discussed above, one of the core challenges is to generate reasonable captions $\tv$ for image $y$. Inspired by previous works \cite{li2023blip,li2024improving}, STiTch aims to solve this with MLLMs due to their impressive performance in image-text understanding. More specifically, here we explore the in-context learning of MLLM and complete the prompt template: ``\textit{$<$in-context prompt$>$. $<x>$. Instruction:$<m>$. Edited Description:}''. Where \textit{$<$in-context prompt$>$} helps MLLMs understand the CIR task and output the expected target descriptions. $<x>$, $<m>$ are the placeholder of the reference image and text modification. 

Intuitively, there are likely several plausible $t$ for each $x$ and $m$ pair, they describe the same target image from different views, To simulate such an ability, we explore the uncertainty generation of MLLMs via sampling from the language model's decoder, to replace the naive greedy decoding used in previous single target description generations. Formally, we combine the top-k and top-p sampling strategy in ~\citep{holtzman2019curious} and collect $K$ possible target description $t$ with a discrete distribution:
\begin{equation}\label{P_t}
    P_t = \frac{1}{K}\sum_{k=1}^K \delta_{\tv_k},
\end{equation}
where $\delta_{\tv}$ refers to a point mass located at coordinate $\tv$, and $\tv_k$ denotes the text embedding of $k$-th generated description. $P_t$ can be viewed as a semantic set containing $K$ reasonable descriptions, and it thus considers diverse visual features of the target image. 
%This probabilistic formulation enables our model to retrieve using different composition knowledge, resulting in robust prediction performance.

\vspace{2mm}
\noindent \textbf{Semantic Transition.} Another challenge comes from the semantic gap between the generated description $t$ and the target image $y$. Generally, an ideal $t$ should highlight the semantic changes while avoiding unnecessary information instructions from the reference image. 
On one hand, we empirically find that existing LLM-based generators can successfully describe the changed context. On the other hand, they also pay more attention to the reference image due to the limited guidance in text modification $m$. As a result, the output caption usually contains many visual details of the reference image, which act as noise and mislead the retrieval process. To this end, we propose a transition step that pushes the generated captions to the target image at the embedding space. 
As shown in Fig.~\ref{framework}, let $\Delta \mv$ denote the difference between $\xv$ and $\yv$, it provides incremental semantics from the reference image to its target. Recalling that the text modification $m$ contains high-quality relative information, it is natural to estimate $\Delta \mv$ using $m$:
\begin{equation}\label{Delta}
    \Delta \mv = \yv - \xv 
    % \approx f(m)
    , 
     \Delta \hat{\mv} = f(m) ,
\end{equation}
where $\xv \in R^d$ represents the visual embeddings of the reference image $x$ generated by the CLIP image encoder, $f$ is the CLIP text encoder. Once obtaining the relative guidance $\Delta \hat{\mv}$, $\tv_k$ can be updated via a simple fusing strategy:
\begin{equation}\label{P_tv2}
    \hat{\tv}_k = (1-\alpha) \tv_k + \alpha \Delta \hat{\mv},
\end{equation}
where the first term $\tv_k$ comes from the MLLMs, and it encodes multimodal knowledge based on the MLLM's understanding of the composed input $(x, m)$. The second term $\Delta \hat{\mv}$ is derived from the text modification estimation and contains high-quality relative instruction between the reference and target image. The transferred caption $\hat{\tv}_k$ takes guidance from both directions with a trade-off hyperparameter $\alpha \in [0,1]$. Now, we can rewrite $P_t$ as: $P_t = \frac{1}{K}\sum_{k=1}^K \delta_{\hat{\tv}_k}$.  
%Higher $\delta$ means we focus more on the relative instruction, and $\delta=0$ denotes no transition step. Now, we can rewrite $P_t$ as:
%\begin{equation}
%    P_t = \frac{1}{K}\sum_{k=1}^K \delta_{\hat{\tv}_k}.
%\end{equation}

\vspace{2mm}
\noindent \textbf{Set-to-set Alignment.} Given the collected discrete distribution $P_t$ in the text domain, we in this section aim to explore the diverse visual features in the image domain with a similar motivation:
%Inspired by previous studies, we formulate the target image as a discrete distribution using various image augmentation tools:
\begin{equation}\label{Q_y}
    Q_y = \frac{1}{M}\sum_{m=1}^M \delta_{{\yv}_m},
\end{equation}
where we augment the target image $M-1$ times and $\{\yv_m\}_{m=2}^{M}$ are the embeddings of the augmented images.
% $m$-th augmentation . 
Unlike previous ZS-CIR models that view the target image as a single point, $Q_y$ in Eq.~\ref{Q_y} provides us with multiple views of $y$, leading to the following fine-grained retrieval strategy. 

Moving beyond the point-to-point similarity measurement in Eq.~\ref{clip}, we here develop a bidirectional distance of two discrete distributions $\mathcal{L}_{bi}(P_t, Q_y)$ under the 
% conditional transport 
CT
framework. Specifically, $\mathcal{L}_{bi}$ consists of two transport costs: the forward cost that measures the expected transport cost from the refined captions to the target image and the backward cost that inverses the direction:
\begin{equation}\label{lbi}
\begin{aligned}
    \mathcal{L}_{bi}(P_t, Q_y) &= \mathcal{L}_{P_t\rightarrow Q_y}(P_t, Q_y) + \mathcal{L}_{Q_y \rightarrow P_t}(P_t, Q_y) \\
    &= \sum_{m,k} \pi(\yv_m|\hat{\tv}_k)c(\hat{\tv}_k,\yv_m) + \pi(\hat{\tv}_k|\yv_m)c(\yv_m,\hat{\tv}_k),
\end{aligned}
\end{equation}
where the cost function $c(\yv,\hat{\tv})=c(\hat{\tv},\yv)$ is specified as the cosine distance to measure the transport cost between points $\hat{\tv}$ and $\yv$. $\pi(\yv|\hat{\tv})$ denotes the transport plan in the forward path, and it measures how likely $\hat{\tv}$ will be transported to $\yv$:
\begin{equation}
    \pi(\yv_m|\hat{\tv}_k) = \frac{\text{exp}(\hat{\tv}_k^T\yv_m / \tau)}{\sum_{m'=1}^M \text{exp}(\hat{\tv}_k^T\yv_{m'} / \tau)}.
\end{equation}
Naturally, the closer $\hat{\tv}$ and $\yv$ are in the embedding space, the higher the transport probability from $\hat{\tv}$ to $\yv$. $\pi(\hat{\tv}|\yv)$ is defined in a similar way:
\begin{equation}
    \pi(\hat{\tv}_k|\yv_m) = \frac{\text{exp}(\yv_m^T\hat{\tv}_k / \tau)}{\sum_{k'=1}^K \text{exp}(\yv_m^T\hat{\tv}_{k'} / \tau)}.
\end{equation}
Mathematically, $\mathcal{L}_{bi}$ in Eq.~\ref{lbi} calculates the distance between two discrete distributions in both forward and backward directions.  This benefits the alignment across the vision and language domains, showing better multimodal retrieval ability. Moreover, $\mathcal{L}_{bi}$ views the generated caption and target image as two discrete distributions, which show great potential in modeling diverse semantics.

Once obtain the bidirectional distance between the generated descriptions and the target image, we can rewrite Eq.~\ref{clip} with $\mathcal{L}_{bi}$, resulting in a more general and fine-grained prediction score:
\begin{equation}\label{qta}
    p(y=i|x,m) = \frac{\text{exp}(-\mathcal{L}_{bi}(P_t, Q_{y_i}))}{\sum_{n=1}^N \text{exp}(-\mathcal{L}_{bi}(P_t, Q_{y_n})}.
\end{equation}
We summarize the whole inference algorithm of STiTch in the Alg.{\color{cvprblue}1}
% ~\ref{alg}
in \pk{Appendix}.
% Alg.~\ref{algo}


==> pvrxdxhprxfbkgzgdcbcvhwnphknnwwq/sec/4_experiment.tex <==
\section{Experiments}
\label{sec:experiment}
% We conduct extensive results on several CIR benchmarks to evaluate the performance of STiTch against the state-of-the-art ZS-CIR models.

\subsection{Experimental Setup}
\paragraph{Datasets.} Following previous works~\cite{tang2025reason}, we evaluate our proposed model on four commonly used CIR datasets, which vary in CIR tasks, image domains and dataset sizes, including CIRR~\cite{liu2021image}, CIRCO~\cite{baldrati2023zero}, FashionIQ~\cite{wu2021fashion}, and GeneCIS~\cite{vaze2023genecis}. CIRR is the first natural image dataset for CIR. CIRCO comes from COCO2017~\cite{lin2014microsoft} and has multiple ground truths for each query. FashionIQ focuses on fashion-related retrieval and consists of three subsets: shirt, dress, and toptee. GeneCIS contains images from MS-COCO~\cite{lin2014microsoft} and Visual Attributes in the Wild~\cite{pham2021learning}, offering four task variations around objects and attributes. We report the original benchmark metrics for each dataset: \textit{e.g.}, Recall@k(R@k) for CIRR, GeneCIS, and FashionIQ, and mean average precision (mAP@k) for CIRCO due to its multiple labels. 

\vspace{2mm}
\noindent \textbf{Baselines.} We compare our STiTch with recent advances, grouped as training-dependent and training-free models. The former often optimize a mapping network to project the reference image into text tokens, including 1) \textbf{Pic2Word}~\cite{saito2023pic2word}, 2) \textbf{SEARLE}~\cite{baldrati2023zero}, 3) \textbf{Context-I2W}~\cite{tang2024context}, and 4) \textbf{LinCIR}~\cite{gu2023language}. Training-free methods focus more on improving ZS-CIR with large language models, including 5) \textbf{CIReVL}~\cite{karthik2023vision}, 6) \textbf{LDRE}~\cite{yang2024ldre}, 7) \textbf{OSrCIR}~\cite{tang2025reason} and 8) \textbf{SEIZE}~\cite{yang2024semantic}. Unlike previous training-free methods, our STiTch aims to refine the composed caption in the embedding space and explore fine-grained alignment across vision-language domains. For all training-based baselines, we directly report the results according to their official papers. For training-free models, to make a fair comparison, we reproduce their results on the FashionIQ dataset according to their released codes and report results on other datasets according to the original papers. We encourage readers to \pk{Appendix} for more details.

\begin{table*}[!t]
\centering
\caption{\small{Comparison on CIRCO and CIRR datasets. The top two training-free results are highlighted in \textbf{bold} and \underline{underline}, respectively. 
% More comparisons are reported in the \pk{Appendix}.
}}
%(*) denotes that we rerun the experiments using their official codes by loading the same ViT-L/14 weights. We also report the comparison with OpenCLIP weights in the Appendix.}}
\label{circo_table}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{c|c|c|cccc||ccc|ccc}
\toprule
\multicolumn{3}{c}{\textbf{CIRCO + CIRR $\rightarrow$}} & \multicolumn{4}{c}{\textbf{CIRCO}} & \multicolumn{6}{c}{\textbf{CIRR}} \\
\hline
\multicolumn{3}{c}{Metric} & \multicolumn{4}{c}{mAP@k} & \multicolumn{3}{c}{Recall@k} & \multicolumn{3}{c}{$\text{Recall}_{\text{Subset}}$@k} \\
Arch & Method & Train & k=5 & k=10 & k=25 & k=50 & k=1 & k=5 & k=10 & k=1 & k=2 & k=3 \\
\hline
\multirow{7}{*}{ViT-L/14}  
%\multirow{9}{*}{ViT-L/14} 
& Pic2Word & \textcolor{red}{\ding{51}} & 8.72 & 9.51 & 10.64 & 11.29 & 23.90 & 51.70 & 65.30 & 53.76 & 74.46 & 87.08 \\
& SEARLE & \textcolor{red}{\ding{51}} & 11.68 & 12.73 & 14.33 & 15.12 & 24.24 & 52.48 & 66.29 & 53.76 & 75.01 & 88.19 \\
& LinCIR & \textcolor{red}{\ding{51}} & 12.59 & 13.58 & 15.00 & 15.85 & 25.04 & 53.25 & 66.68 & 57.11 & 77.37 & 88.89 \\
& Context-I2W & \textcolor{red}{\ding{51}} & 13.04 & 14.62 & 16.14 & 17.16 & 25.60 & 55.10 & 68.50 & - & - & - \\
& CIReVL & \textcolor{green}{\ding{55}} & 18.57 & 19.01 & 20.89 & 21.80 & 24.55 & 52.31 & 64.92 & 59.54 & 79.88 & 89.69    \\
% & CIReVL\textsuperscript{*}\tiny{[ICLR'24]} & \textcolor{green}{\ding{55}} & 18.92 & 19.32 & 21.15 & 22.14 & 24.83 & 52.68 & 65.28 & 59.82 & 80.15 & 89.98 \\
& LDRE & \textcolor{green}{\ding{55}} & 23.35 & 24.03 & 26.44 & 27.50 & 26.53 & 55.57 & 67.54 & 60.43 & 80.31 & 89.90 \\
% & OSrCIR & \textcolor{green}{\ding{55}} & 30.47 & 31.14 & 35.03 & 36.59 & 37.26 & 67.25 & 77.33 & 69.22 & 85.28 & 93.55 \\
& OSrCIR & \textcolor{green}{\ding{55}} & {23.87} & {25.33} & {27.84} & \underline{28.97} & \textbf{29.45} & \underline{57.68} & \underline{69.86} & {62.12} & {81.92} & {91.10} \\
& SEIZE & \textcolor{green}{\ding{55}} & \underline{24.98} & \underline{25.82} & \underline{28.24} & 28.35 & 28.65 & 57.16 & 69.23 & \underline{62.22} & \underline{84.05} & \underline{92.34} \\
% & \textbf{Ours} & \textcolor{green}{\ding{51}} & 21.74 & 22.90 & 25.30  & 26.37\\
% & \textbf{Ours (AWT)} & \textcolor{green}{\ding{51}} & \\
& \cellcolor{gray!20} \textbf{STiTch(Ours)} & \cellcolor{gray!20}\textcolor{green}{\ding{55}} &  \cellcolor{gray!20}\textbf{25.55} & \cellcolor{gray!20}\textbf{26.27} & \cellcolor{gray!20}\textbf{28.81} & \cellcolor{gray!20}\textbf{29.99} & \cellcolor{gray!20}\underline{28.87} & \cellcolor{gray!20}\textbf{57.97} & \cellcolor{gray!20}\textbf{69.90} & \cellcolor{gray!20}\textbf{65.22} & \cellcolor{gray!20}\textbf{84.10} & \cellcolor{gray!20}\textbf{92.37}\\
\midrule
\multirow{3}{*}{ViT-G/14}
& CIReVL & \textcolor{green}{\ding{55}} & 26.77 & 27.59 & 29.96 & 31.03 & 34.65 & 64.29 & 75.06 & 67.95 & 84.87 & 93.21 \\
%CIReVL & \textcolor{green}{\ding{55}} & 27.12 & 28.01 & 30.35 & 31.39 & 34.98 & 64.68 & 75.41 & 68.37 & 85.23 & 93.24 \\
% &Slerp & \textcolor{green}{\ding{55}} & 31.12 & 32.24 & 34.95 & 36.03 & 36.15 & 66.39 & 77.25 & 68.82 & 85.66 & 93.76 \\
& LDRE & \textcolor{green}{\ding{55}} & {31.12} & {32.24} & 34.95 & 36.03 & 36.15 & 66.39 & 77.25 & 68.82 & {85.66} & {93.76} \\
& OSrCIR & \textcolor{green}{\ding{55}} & 30.47 & 31.14 & {35.03} & {36.59} & {37.26} & {67.25} & {77.33} & {69.22} & 85.28 & 93.55 \\
& SEIZE & \textcolor{green}{\ding{55}} & \underline{32.46} & \underline{33.77} & \underline{36.46} & \underline{37.55} & \underline{38.87} & \underline{69.42} & \underline{79.42} & \textbf{74.15} & \underline{89.23} & \underline{95.71} \\
% & \textbf{Ours} & \textcolor{green}{\ding{51}} & 32.46 & 33.90 & 36.75 & 37.96 & \\
% & \textbf{Ours (AWT)} & \textcolor{green}{\ding{51}} & \\
& \cellcolor{gray!20} \textbf{STiTch (Ours)} & \cellcolor{gray!20}\textcolor{green}{\ding{55}} & \cellcolor{gray!20}\textbf{34.40} & \cellcolor{gray!20}\textbf{35.56} & \cellcolor{gray!20}\textbf{38.07} & \cellcolor{gray!20}\textbf{40.02} & \cellcolor{gray!20}\textbf{39.23} & \cellcolor{gray!20}\textbf{69.95} & \cellcolor{gray!20}\textbf{79.56} & \cellcolor{gray!20}\underline{73.56} & \cellcolor{gray!20}\textbf{89.50} & \cellcolor{gray!20}\textbf{95.86} \\
\bottomrule
\end{tabular}}
\vspace{-3mm}
\end{table*}

\vspace{2mm}
\noindent \textbf{Implementation Details.} We employ the open-source Qwen2-VL-7B as our MLLM by default, while we also report the results on various MLLMs in {\pk{Appendix} 
% \ref{appendix_sec_mllm}
{\color{cvprblue}C}
}. To generate diverse descriptions, we follow a similar setting to previous works and apply $\tau=0.7$, top-k(k=50), top-p(p=0.8) at the querying stage. Regarding image augmentation, we used only random resized crop and random horizontal flip for each image. We set the number of captions as $K=5$, the number of augmentations as $M=10$, and employ a default value of $\alpha=0.45$. The default retrieval model is CLIP-L/14 from the official OpenAI implementation~\cite{radford2021learning}. We also report the results of LLM-based models (CIReVL, OSrCIR, and our STiTch) on CLIP-bigG-14 from the OpenCLIP implementation~\cite{cherti2023reproducible} for analysis of scaling laws.
All experiments are conducted on a single NVIDIA A6000 GPU.



\subsection{Comparison with State-of-the-art Methods}
We run all experiments three times with different random seeds and report the mean value to ensure reliability. We report the comparison on the hidden test set of CIRCO and CIRR datasets in Tab.~\ref{circo_table} (All results are obtained from the submission server provided in \cite{baldrati2023zero} and \cite{liu2021image}). These two CIR datasets focus on foreground and background differentiation and fine-grained image editing. From the results, we find that our proposed STiTch achieves the best or second-best results in most cases among baselines, including training-free and textual inversion models. STiTch underperforms baselines on the CIRR dataset in the case of $k=1$. This may be due to the noisy annotation in CIRR, where the reference image is less related to the target image~\cite{baldrati2023zero}. 
% When considering the subset retrieval setting ($\text{Recall}_{Subset}$), where the correct image has to be retrieved from 6 curated images, our STiTch beats OSrCIR by achieving a significant improvement. For example, STiTch achieves $3.26\%$, $2.72\%$ and $1.61\%$ relative improvements in $k=1$,$k=2$ and $k=3$ settings {on CLIP-G-14}, respectively. More comparisons are reported in the Appendix Tab.~\ref{appendix_c}.


\begin{table*}[!t]
\centering
\caption{\small{Comparison on Fashion-IQ datasets. The top two training-free results are highlighted in \textbf{bolded} and \underline{underlined}. 
% More results with different backbones are reported in Tab.~\ref{appendix_f}.}}
% More comparisons are reported in the \pk{Appendix}.
}}
\vspace{-2mm}
\label{fashioniq}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|c|c|cccccc|cc}
\toprule
\multicolumn{3}{c}{\textbf{Fashion-IQ $\rightarrow$}} & \multicolumn{2}{c}{\textbf{Shirt}} & \multicolumn{2}{c}{\textbf{Dress}} & \multicolumn{2}{c}{\textbf{Toptee}} & \multicolumn{2}{c}{\textbf{Average}} \\
\hline
Arch & Method & Train & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 & R@10 & R@50 \\
\hline
\multirow{6}{*}{ViT-G/14} 
& Pic2Word & \textcolor{red}{\ding{51}} & 33.17 & 50.39 & 25.43 & 47.65 & 35.24 & 57.62 & 31.28 & 51.89 \\
& SEARLE & \textcolor{red}{\ding{51}} & 36.46 & 55.35 & 28.16 & 50.32 & 39.83 & 61.45 & 34.81 & 55.71 \\
& LinCIR & \textcolor{red}{\ding{51}} & {46.76} & {65.11} & {38.08} & {60.88} & {50.48} & {71.09} & {45.11} & {65.69} \\
& CIReVL & \textcolor{green}{\ding{55}} &  29.85 & 51.07 & 27.07 & 49.53 & 35.80 & 56.14 & 32.19 & 52.36 \\
% & CIReVL* & \textcolor{green}{\ding{55}} & 31.65 & 49.07 &  23.90 & 43.13 & 32.53 & 53.19 & 29.36 & 48.46\\
% & CIReVL\dag & \textcolor{green}{\ding{55}} & 32.63 & 50.05 & 25.09 & 45.12 & 34.42 & 55.12 & 30.71 & 50.10 \\
% & CIReVL\textsuperscript{*}\tiny{[ICLR'24]} & \textcolor{green}{\ding{55}} & 34.01 & 51.92 & 27.56 & 50.04 & 36.29 & 56.63 & 32.62 & 52.86 \\
% & LDRE & \textcolor{green}{\ding{55}} & 35.94 & \textbf{58.58} & 26.11 & 51.12 & 35.42 & 56.67 & 32.49 & 55.46 \\
& OSrCIR & \textcolor{green}{\ding{55}} & {{38.65}} & {54.71} & {33.02} & {54.78} & {41.04} & {61.83} & {37.57} & {57.11} \\
% & OSrCIR* & \textcolor{green}{\ding{55}}  & 36.56 & 55.45 & 30.69 & 53.25 & 40.13 & 61.30 & 35.79 & 56.67\\
% & OSrCIR\dag & \textcolor{green}{\ding{55}}  & 37.39 & 56.92 & 30.59 & 53.50 &  39.72 & 61.04 & 35.79 & 57.15 \\
& SEIZE & \textcolor{green}{\ding{55}} & \textbf{43.60} & \textbf{65.42} & \textbf{39.61} & \textbf{61.02} & \textbf{45.94} & \textbf{71.12} & \textbf{43.05} & \textbf{65.85} \\
% & \textbf{Ours} & \textcolor{green}{\ding{55}} & 36.36 & 55.50 & 32.28 & 54.14 & 38.55 & 62.01 & 35.73 & 57.21  \\
% & \textbf{Ours (AWT)} & \textcolor{green}{\ding{55}} & 38.27 & 57.41 & 31.78 & 52.26 & 41.00 & 63.28 & 37.01 & 57.65 \\
% & Ours (CT) & \textcolor{green}{\ding{55}} & 37.44 & 56.82 & 30.24 & 52.65 & 40.13 & 62.21 & 35.93 & 57.23 \\
& \cellcolor{gray!20}\textbf{STiTch(Ours)} & \cellcolor{gray!20}\textcolor{green}{\ding{55}} & \cellcolor{gray!20}{\underline{39.48}}  & \cellcolor{gray!20}{\underline{56.59}} & \cellcolor{gray!20}{\underline{35.04}} & \cellcolor{gray!20}{\underline{56.74}} & \cellcolor{gray!20}{\underline{42.86}} & \cellcolor{gray!20}{\underline{64.95}} & \cellcolor{gray!20}{\underline{39.12}} &  \cellcolor{gray!20}{\underline{59.43}} \\
\bottomrule
\end{tabular}}
\end{table*}



\begin{table*}[!t]
\centering
\caption{\small{Comparison on GeneCIS datasets. The top two training-free results are highlighted in \textbf{bolded} and \underline{underlined}, respectively.}}
\vspace{-2mm}
\label{genecis}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|cccccccccccc|c}
\toprule
\multicolumn{3}{c}{\textbf{GeneCIS $\rightarrow$}} & \multicolumn{3}{c}{\textbf{Focus Attribute}} & \multicolumn{3}{c}{\textbf{Change Attribute}} & \multicolumn{3}{c}{\textbf{Focus Object}} & \multicolumn{3}{c}{\textbf{Change Object}} & \multicolumn{1}{c}{\textbf{Average}}  \\
\hline
Arch & Method & Train & R@1 & R@2 & R@3 & R@1 & R@2 & R@3 & R@1 & R@2 & R@3 & R@1 & R@2 & R@3 & R@1 \\
\hline
\multirow{7}{*}{ViT-L/14} 
& SEARLE & \textcolor{red}{\ding{51}} & 17.1 & 29.6 & 40.7 & 16.3 & 25.2 & 34.2 & 12.0 & 22.2 & 30.9 & 12.0 & 24.1 & 33.9 & 14.4 \\
& LinCIR & \textcolor{red}{\ding{51}} & 16.9 & 30.0 & 41.5 & 16.2 & 28.0 & 36.8 & 8.3 & 17.4 & 26.2 & 7.4 & 15.7 & 25.0 & 12.2 \\
& Context-I2W & \textcolor{red}{\ding{51}} & 17.2 & 30.5 & 41.7 & 16.4 & 28.3 & 37.1 & 8.7 & 17.9 & 26.9 & 7.7 & 16.0 & 25.4 & 12.7\\
& CIReV & \textcolor{green}{\ding{55}} & 19.5 & 31.8 & 42.0 & 14.4 & 26.0 & 35.2 & 12.3 & 21.8 & 30.5 & 17.2 & 28.9 & 37.6 & 15.9\\
%& CIReVL\textsuperscript{*}\tiny{[ICLR'24]} & \textcolor{green}{\ding{55}} & 19.7 & 32.1 & 42.3 & 14.8 & 26.2 & 35.4 & 12.5 & 22.1 & 30.7 & 17.3 & 29.1 & 37.9 & 16.1\\
& OSrCIR & \textcolor{green}{\ding{55}} & \textbf{20.9} & {33.1} & {44.5} & {17.2} & {28.5} & {37.9} & {15.0} & {23.6} & {34.2} & {18.4} & {30.6} & {38.3} & {17.9} \\
& SEIZE & \textcolor{green}{\ding{55}} & \underline{20.5} & \underline{33.4} & \underline{45.0} & \underline{17.6} & \underline{28.9} & \underline{38.5} & \underline{15.4} & \underline{25.6} & \underline{36.2} & \underline{18.7} & \underline{30.9} & \underline{39.8} & \underline{18.1} \\
% & \textbf{Ours} & \textcolor{green}{\ding{55}} & 19.6 & 32.7 & 43.1 & 17.1 & 29.6 & 39.4 & 16.8 & 27.8 & 37.6 & 18.9 & 30.7 & 40.6 & 18.1 \\
% & \textbf{Ours (AWT)}  & \textcolor{green}{\ding{55}} & 20.6 & 34.5 & 45.8 & 18.0 & 29.2 & 40.3 & 16.8 & 27.9 & 38.2 & 18.8 & 30.2 & 40.1 & 18.5 \\
& \cellcolor{gray!20}\textbf{STiTch(Ours)} & \cellcolor{gray!20}\textcolor{green}{\ding{55}} &\cellcolor{gray!20}\uline{20.3} & \cellcolor{gray!20}\textbf{34.6} & \cellcolor{gray!20}\textbf{46.4} & \cellcolor{gray!20}\textbf{18.3} & \cellcolor{gray!20}\textbf{29.8} & \cellcolor{gray!20}\textbf{41.6} & \cellcolor{gray!20}\textbf{16.8} & \cellcolor{gray!20}\textbf{28.5} & \cellcolor{gray!20}\textbf{38.4} & \cellcolor{gray!20}\textbf{18.8} & \cellcolor{gray!20}\textbf{31.0} & \cellcolor{gray!20}\textbf{40.3} & \cellcolor{gray!20}\textbf{18.6} \\
\midrule
\multirow{3}{*}{ViT-G/14}
& CIReVL & \textcolor{green}{\ding{55}} & 20.9 & 34.4 & 44.9 & 16.5 & 29.0 & 39.8 & 15.1 & 25.6 & 33.4 & 18.5 & 31.6 & 41.4 & 17.8 \\
& OSrCIR & \textcolor{green}{\ding{55}} & \underline{22.7} & \underline{36.4} & 47.0 & 17.9 & 30.8 & 42.0 & 16.9 & 28.4 & 36.7 & \textbf{21.0} & \textbf{33.4} & \textbf{44.2} & 19.6 \\
& SEIZE & \textcolor{green}{\ding{55}} & \textbf{22.9} & 36.2 & \underline{47.3} & \underline{18.6} & \underline{31.4} & \underline{42.7} & \underline{18.2} & \underline{28.8} & \underline{37.6} & {19.6} & {33.0} & \underline{43.5} & \underline{19.8} \\
& \cellcolor{gray!20}\textbf{STiTch (Ours)} & \cellcolor{gray!20}\textcolor{green}{\ding{55}} &\cellcolor{gray!20}{21.9} & \cellcolor{gray!20}\textbf{36.4} &\cellcolor{gray!20}\textbf{47.9} &\cellcolor{gray!20}\textbf{19.6} &\cellcolor{gray!20}\textbf{31.9} &\cellcolor{gray!20}\textbf{42.8} &\cellcolor{gray!20}\textbf{20.2} &\cellcolor{gray!20}\textbf{30.3} &\cellcolor{gray!20}\textbf{39.6} & \cellcolor{gray!20}\underline{19.7} &\cellcolor{gray!20}\underline{33.2} &\cellcolor{gray!20}\uline{43.4} &\cellcolor{gray!20} \textbf{20.4} \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\end{table*}


Tab.~\ref{fashioniq} shows the comparison in the validation set of the Fashion-IQ dataset with ViT-G/14, and more comparisons on other backbones can be found in the \pk{Appendix} 
% Tab.~\ref{appendix_f}
Tab. {\color{cvprblue}7}. The results show the robustness of our method. Interestingly, we find that text inversion-based models (e.g., LinCIR) outperform LLM-based models in the fashion image editing task. This may be due to the fact that most images in Fashion-IQ are relatively simple, containing only a pure background. This may limit the ability of MLLMs, and in contrast, training-dependent models tend to describe the reference image more correctly. 
% \rr{Among LLM-based models, SEIZE achieves the best recall. Both SEIZE and STiTch refine the target captions, where STiTch employs modification text as transition vectors, while SEIZE utilizes generated reference captions to adjust final predictions. We find that the modification text in Fashion-IQ is overly simplistic (\textit{e.g.}, is solid white and is a lighter color), resulting in suboptimal guidance for STiTch. SEIZE relies on a pre-trained caption model to generate reference captions, which may be better suited for Fashion-IQ's simplified scenarios. However, as shown in the Tab.~\ref{efficiency_vs}, this approach increases the computational cost during inference.}

% The simple scenes in FashionIQ make it easy to capture the modification relationship between the reference and target image, which may be more suitable for SEIZE.

% This may be because of its two-stage generation, where the generated reference caption 

% achieves the second recall score on the Dress and Toptee datasets and shows competitive results on the Shirt dataset, demonstrating the effectiveness of the introduced transition-aware bidirectional alignment across vision-language domains.

Lastly, we further test the object and attribute composition ability of our model on the GeneCIS dataset, with the results listed in Tab.~\ref{genecis}. Unlike previous datasets that provide a detailed text modification sentence, GeneCIS uses single-word instruction to express the user's intent, \textit{e.g.}, focusing/changing a specific object or attribute. From the results, we find that our proposed STiTch achieves the best results in 19/24 cases and outperforms the others at the average score. On the one hand, STiTch preserves rich multimodal knowledge to interpret implicit inputs while filtering out noise through transition. On the other hand, it views the caption as a discrete distribution, showing great potential in capturing diverse visual semantics, leading to fine-grained retrieval for this complex task. 
% More comparisons are reported in \pk{Appendix} Tab.
% % ~\ref{appendix_g}
% {\color{cvprblue}8}.

% \vspace{-3mm}
\subsection{Further Analysis}
In addition to the numerical comparisons on four CIR benchmarks. In this section, we provide further analysis of the ablation results and visualizations of the proposed modules.

% on the proposed modules and the visualization of the transferred descriptions.

% \begin{figure}
% \centering
% \includegraphics[width=0.8\linewidth]{figs/Ablation.pdf}
% % \caption{\small{Results of CIRCO and CIRR datasets on CLIP-bigG/14 with various description numbers (a) and target image augmentations (b).}}
% \caption{{\small{
% % Results of CIRCO datasets on CLIP-B/32 with various description numbers and image augmentations.
% Ablation results of the number of descriptions and image augmentations on the CIRCO dataset with CLIP-B/32.}}
% \label{km}}
% \vspace{-5mm}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.73\linewidth]{figs/backbone.pdf}
%     \caption{{\small{
%     % Results of four datasets on CLIP-L/14 with different transport method.
%     Ablation results of different alignment strategies across four datasets with CLIP-L/14.
%     }}
%     \label{ot}}
%     \vspace{-5mm}
% \end{figure}

% \begin{table*}[!t]
% \centering
% \caption{\small{Ablation results on the transition and transportation modules. All results are conducted on CIRCO and CIRR datasets with CLIP-bigG/14.}}
% \label{module_ab_tt}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{cc|cccc||ccc|ccc}
% \toprule
% \multicolumn{2}{c}{\textbf{CIRCO + CIRR $\rightarrow$}} & \multicolumn{4}{c}{\textbf{CIRCO}} & \multicolumn{6}{c}{\textbf{CIRR}} \\
% \hline
% \multicolumn{2}{c}{Strategy} & \multicolumn{4}{c}{mAP@k} & \multicolumn{3}{c}{Recall@k} & \multicolumn{3}{c}{$\text{Recall}_{\text{Subset}}$@k} \\
% \textit{Transition} & \textit{Transportation} & k=5 & k=10 & k=25 & k=50 & k=1 & k=5 & k=10 & k=1 & k=2 & k=3 \\
% \hline
% % CIReVL\tiny{[ICLR'24]} & & & 26.77 & 27.59 & 29.96 & 31.03 & 34.65 & 64.29 & 75.06 & 67.95 & 84.87 & 93.21 \\ STiTch w/o TA STiTch w/o T STiTch w/o A STiTch STiTch w/ OT
% \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & 35.11 & 36.65 & 39.69 & 40.87 & 36.22 & 66.36 & 76.84 & 69.93 & 86.48 & 94.05\\
% \textcolor{green}{\ding{51}} & \textcolor{red}{\ding{55}} & 35.72 & 37.20 & 40.28 & 41.44 & {37.69} & {67.76} & {77.69} & {71.81} & {87.45} & {94.51}\\
% \textcolor{red}{\ding{55}} & \textcolor{green}{\ding{51}} & 35.85 & 37.04 & 39.92 & 41.18 & 36.27 & 67.01 & 76.77 & 70.15 & 86.68 & 94.48 \\
% \textcolor{green}{\ding{51}} & \textcolor{green}{\ding{51}} & \textbf{36.44} & \textbf{37.60} & \textbf{40.65} & \textbf{41.90} & \textbf{37.88} & \textbf{68.10} & \textbf{78.56} & \textbf{72.48} & \textbf{88.00} & \textbf{95.16}\\
% % STiTch w/ OT & & & 33.77 & 35.27 & 38.1 & 39.35 & \uline{37.78} & 67.37 & 77.81 & 72.43 & 87.88 & \uline{94.75}\\
% \bottomrule
% \label{ablation_ta}
% \end{tabular}}
% \vspace{-5mm}
% \end{table*}

% \begin{figure}
% \centering
% \begin{minipage}{0.48\textwidth}
% \centering
% \includegraphics[width=0.8\linewidth]{figs/Ablation.pdf}
% \caption{\small{Ablation on the number of descriptions and image augmentations (Aug-$m$:$m$ augmentations per image) on the CIRCO dataset with CLIP-B/32.}}
% \label{km}
% \end{minipage}\hfill
% \begin{minipage}{0.48\textwidth}
% \centering
% \includegraphics[width=0.8\linewidth]{iclr2026/figs/STiTch_ab_ot.png}
% \vspace{-3mm}
% \caption{\small{Ablation results of different alignment strategies across four datasets with CLIP-L/14.}}
% \label{ot}
% \end{minipage}
% \vspace{-5mm}
% \end{figure}

\vspace{2mm}
\noindent \textbf{Main component analysis.} 
% As discussed above, we in this paper aim to improve MLLM-based ZS-CIR via the introduced semantic transition and transportation modules. 
To evaluate the impacts of each proposed module in STiTch, we report the ablation results in Tab.~\ref{module_ab_tt}. We find that 1) both transition and transportation show a positive improvement compared to the base model (first row, query only); 2) The transition module achieves higher improvements than the transportation module in most cases. This shows the validity of our proposed transition vector 
in assessing
the difference between the reference and target images. It highlights the text modification and offers useful guidance to steer the original caption toward the target image, resulting in more correct alignments. 3) Through collaboration, our complete model achieves the best performance. This highlights the motivation of our STiTch: the unnecessary visual details introduced in original captions and the simple point-based alignment.

\begin{figure}[h]
\centering
\includegraphics[width=0.80\linewidth]{sec/Fig/Ablation.pdf}
\caption{\small{Ablation on the number of descriptions and image augmentations (Aug-$10$: $10$ augmentations per image) on the CIRCO dataset with CLIP-B/32.}}
\label{km}
\vspace{-4mm}
\end{figure}

\vspace{2mm}
\noindent \textbf{Impacts of caption number and augmentation views.} 
{We report the study of caption number $K$ and augmentation views $M$ in Eq.~\ref{Q_y} on CIRCO dataset, with results in Fig.~\ref{km}. 
% to test the impacts of the number of modified captions and image augmentations 
From these results, we first find that the performance shows a large improvement when $K>1$. This demonstrates the effectiveness of using diverse captions, especially after semantic transitions, to capture rich semantic information. Moreover, increasing the number of image augmentations $M$ consistently enhances performance, 
highlighting the value of multi-scale image diversity. We suggest that setting $K = 5$ and $M = 10$ is sufficient to achieve strong performance across most datasets.}

\begin{figure}[h]
\centering
\includegraphics[width=0.80\linewidth]{sec/Fig/ablation_transportation_method.png}
\vspace{-3mm}
\caption{\small{Ablation results of different alignment strategies across four datasets with CLIP-L/14.}}
\label{ot}
\vspace{-4mm}
\end{figure}

\vspace{2mm}
\noindent \textbf{Impacts of the bidirectional distance.} Recalling that we propose to measure the distance between the modified caption $P_t$ and the target image augmentation $Q_y$ using a bidirectional transportation distance in Eq.~\ref{lbi}. This enables the proposed STiTch 
% has the ability 
to not only calculate the transport cost from $P_t$ to $Q_y$ but also consider the reverse cost, showing better alignments across the vision-language domains. {To identify such improvements, we replace the 
% proposed
bidirectional CT distance with the optimal transport (OT) distance and report the comparison on four datasets in Fig.~\ref{ot}.} Note that the CT distance consistently beats the OT distance in all cases, showing the effectiveness of our bidirectional alignment.




\begin{table*}[!t]
\centering
\caption{\small{Ablation results on the transition and transportation modules. All results are conducted on CIRCO and CIRR datasets with CLIP-bigG/14.}}
\label{module_ab_tt}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{cc|cccc||ccc|ccc}
\toprule
\multicolumn{2}{c}{\textbf{CIRCO + CIRR $\rightarrow$}} & \multicolumn{4}{c}{\textbf{CIRCO}} & \multicolumn{6}{c}{\textbf{CIRR}} \\
\hline
\multicolumn{2}{c}{Strategy} & \multicolumn{4}{c}{mAP@k} & \multicolumn{3}{c}{Recall@k} & \multicolumn{3}{c}{$\text{Recall}_{\text{Subset}}$@k} \\
\textit{Transition} & \textit{Transportation} & k=5 & k=10 & k=25 & k=50 & k=1 & k=5 & k=10 & k=1 & k=2 & k=3 \\
\hline
\textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & 31.23 & 32.87 & 36.32 & 38.04 & 37.22 & 67.36 & 77.84 & 69.93 & 86.48 & 94.05\\
\textcolor{red}{\ding{51}} & \textcolor{red}{\ding{55}} & 31.89 & 34.46 & 37.94 & 39.67 & {38.33} & {68.45} & {78.03} & {72.81} & {88.13} & {94.51}\\
\textcolor{red}{\ding{55}} & \textcolor{red}{\ding{51}} & 32.14 & 34.78 & 37.87 & 39.48 & 38.48 & 68.38 & 78.34 & 72.15 & 88.04 & 94.48 \\
\textcolor{red}{\ding{51}} & \textcolor{red}{\ding{51}} & \textbf{34.40} & \textbf{35.56} & \textbf{38.07} & \textbf{40.02} & \textbf{39.23} & \textbf{69.95} & \textbf{79.56} & \textbf{73.56} & \textbf{89.50} & \textbf{95.86}\\
% STiTch w/ OT & & & 33.77 & 35.27 & 38.1 & 39.35 & \uline{37.78} & 67.37 & 77.81 & 72.43 & 87.88 & \uline{94.75}\\
\bottomrule
\label{ablation_ta}
\end{tabular}}
\vspace{-2mm}
\end{table*}

\begin{figure*}[!t]
\centering
\includegraphics[width=0.97\textwidth]{sec/Fig/vis_v3_stt.pdf} %{figs/vis_v8.pdf}
% \vspace{-3mm}
\caption{{\small{
Visualization of the GeneCIS dataset on the 'Focus Object' task. Heatmaps before and after the transition on target image are shown. Captions generated by MLLMs often contain irrelevant visual noise (\textit{\sky{blue}} text), while the STiTch model effectively suppresses such noise and highlights the correct focus object (\textit{\rr{red}} text).
}}
\label{vis}}
\end{figure*}

\begin{table*}[!t]
\setlength{\tabcolsep}{8pt} % 缩小列间距
\renewcommand{\arraystretch}{0.7} % 缩小行间距
\centering
\caption{\small{Efficiency comparison with SOTA methods. Inference times (seconds per query) are reported for each model using a single NVIDIA A6000 GPU.}}
\label{efficiency_vs}
\scalebox{0.9}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model} & Pic2Word & SEARLE & CIReVL & OSrCIR & LDRE &SEIZE & STiTch \\
\midrule
\textbf{Time (s)} & $<$0.01 & $<$0.01 & 2.97+0.85=3.82 & 6.65 & 1.30+2.98=4.28 &5.8+4.5=10.3 & 3.5 \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\end{table*}

\vspace{1.5mm}
\noindent \textbf{Visualization Analysis.} From the above analysis, we find that the transition module plays a key role in improving the CIR performance. It estimates the relative vector as the difference between the reference and target image and provides correct information to refine the generated captions. To make a clearer understanding, we visualize the heat maps of two samples from the GeneCIS dataset on the ``Focus Object" task in Fig.~\ref{vis}. Here, we directly calculate the cosine similarity between the visual patch embeddings and the caption embedding as the score of the heat maps. The first row denotes three generated captions and the last two heat maps denote the corresponding visualization results before and after the transition module. We find that the generated captions indeed introduce visual noise for the CIR task. For example, the retrieval attentions are often disturbed by visual noise such as ``white fence", ``white color" and ``left side of the scene". In contrast, the visualizations of STiTch often focus on the correct object, leading to higher CIR performance. 


\vspace{1.5mm}
\noindent \textbf{Efficiency Analysis.} Tab. \ref{efficiency_vs} shows the inference times (seconds per query) of various methods. Overall, LLM-based methods generally incur higher test-time latency than traditional mapping models due to the query stage. For instance, CIReVL, LDRE and SEIZE are two-stage approaches that require significant time to generate target descriptions, while OSrCIR involves extensive chain-of-thought reasoning during inference. In contrast, our STiTch achieves the lowest test time among LLM-based methods when taking image augmentation into consideration, showing the efficiency of our collaborative modules. 





==> pvrxdxhprxfbkgzgdcbcvhwnphknnwwq/sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we propose STiTch, a novel one-stage, training-free framework for the zero-shot composed image retrieval task. STiTch improves the quality of the generated caption by MLLMs via a transition vector and views the captions and target image as two discrete distributions in the embedding space. A bidirectional transport distance is developed to measure the similarity across the vision-language domains. Our approach not only achieves strong performance on four CIR benchmarks but also, provides interpretability via the visualization of the transferred caption and the target images. Extensive ablations also demonstrate the effectiveness of STiTch. Since its natural flexibility and simplicity, we hope STiTch provides innovative ideas for follow-up studies.

\clearpage
\subsection*{Acknowledgments}
This research was supported in part by the Hong Kong RGC General Research Fund (Grant Nos. 15221123, 15216424, and 15211525) and the PolyU Internal Research Fund (Grant Nos. P0058468 and P0056171); in part by the Young Scientists Fund of the National Natural Science Foundation of China (Grant No. 62506237); in part by the National Natural Science Foundation of China (Grant No. 62576215); and in part by the Scientific Foundation for Youth Scholars of Shenzhen University.
% This research was supported by funding from the 
% Hong Kong RGC General Research Fund (No. 152211/23E, 15216424/24E, and 152115/25E), the PolyU Internal Fund (No. P0056171), and the Huawei Gifted Fund.
